$G_2$-instantons over asymptotically cylindrical manifolds

A concrete model for a 7-dimensional gauge theory under special holonomy is proposed, within the paradigm outlined by Donaldson and Thomas, over the asymptotically cylindrical G2-manifolds provided by Kovalev's noncompact version of the Calabi conjecture. One obtains a solution to the $G_2$-instanton equation from the associated Hermitian Yang-Mills problem, to which the methods of Simpson et al. are applied, subject to a crucial asymptotic stability assumption over the "boundary at infinity".

==> EACCY_3-fold.tex <==

%MINHAS FIGURAS

\setlength{\unitlength}{0.5cm}

%FIGURA ESQUERDA
\begin{picture}(0,8.5)(-3,-4)

%ORIGEM
%\put(0,0){\circle*{0.2}}\put(-1,-0.5){(0,0)}

%QUADRICULADO
%\multiput(0,-5)(1,0){13}{\line(0,1){12}}
%\multiput(0,-5)(0,1){13}{\line(1,0){15}}

\put(1.5,-5){\huge{$W_0$}}


\linethickness{0.4mm}

%CURVA CONTINUA
%%CIMA
\qbezier(4,2)   (3,3)
        (2,3)

\qbezier(4,2)   (5,1)
        (6,1)

%%BAIXO
\qbezier(2,-3)  (3,-3)
        (4,-2)
\qbezier(4,-2)   (5,-1)
        (6,-1)


%LATERAL
\qbezier(2,3)(0,3)
        (0,0)
\qbezier(0,0)(0,-3)
        (2,-3)

%TUBO
\put(9,1){\line(-1,0){3}}
\put(9,-1){\line(-1,0){3}}

\put(9.5,0){\dots}

\put(12,1){\line(-1,0){1}}
\put(12,-1){\line(-1,0){1}}


%W_\infty
\linethickness{0.1mm}
\put(9,-5){\huge{$W_\infty$}}
\multiput(6,-5.5)(0,0.5){8}{\line(0,1){0.25}}

%SECAO TRANSVERSAL

%%W_0

\qbezier(6,1)  (7,0)
        (6,-1)


\linethickness{0.4mm}

\qbezier(6,1)  (5,0)
        (6,-1)

%%bordo de W_S

\linethickness{0.7mm}
\qbezier(12,1)  (11,0)
        (12,-1)


\qbezier(12,1)  (13,0)
        (12,-1)

\put(12.8,-2.5){$\partial W_S$}

%EIXO S
\put(4.93,3){
\[\xy(0,0);<0.5cm,0cm>:
        \ar@{|->} 0*^+!DR{0};p+(10,0) *^+!DL{s} ^(.6)*@{|} _(.6)*[o]+{S}
\endxy\]
}

%

%BORDO
\put(13.25,0){$\simeq$}
\put(14.2,0.8){
\[\xy(0,0);<0.4cm,0cm>:
%%SUPERFICIE D
        (2,0)*{\txt\small\itshape{D}}="D",
        (-1,0);(1,0) **\crv{(0,1)},
        (-1,0);(0,-0.5) **\crv{(0,0)},
        (0,-0.5);(1,0) **\crv{(0,0)},
        %
        (0.04,-1.15) *{^\times},
        %
%%S1 ALPHA
        (2,-2) *{\txt\small\itshape{S}};p+(0.6,0)*{^1},
        (0,-1.5);(0,-2.5) **\crv{(0.5,-2)},
        ?(0.9)*!/^0.2mm/{\txt{ \^}},
        (0,-1.5);(0,-2.5) **\crv{(-0.5,-2)},
        %
        \endxy\]
}

\end{picture}





